Testing GLOM's ability to infer wholes from ambiguous parts

The GLOM architecture proposed by Hinton [2021] is a recurrent neural network for parsing an image into a hierarchy of wholes and parts. When a part is ambiguous, GLOM assumes that the ambiguity can be resolved by allowing the part to make multi-modal predictions for the pose and identity of the whole to which it belongs and then using attention to similar predictions coming from other possibly ambiguous parts to settle on a common mode that is predicted by several different parts. In this study, we describe a highly simplified version of GLOM that allows us to assess the effectiveness of this way of dealing with ambiguity. Our results show that, with supervised training, GLOM is able to successfully form islands of very similar embedding vectors for all of the locations occupied by the same object and it is also robust to strong noise injections in the input and to out-of-distribution input transformations.

==> exp2.tex <==


\subsection{Basic Experiment}



Three experimental set-ups are explored: a single object (either a Face or a Sheep) in an input, two objects (either a face or a sheep) in an input, and two objects in an input, where the objects are one of twenty randomly generated object types.  Fig. ~\ref{fig:example_outputs} shows that the whole objects are able to be predicted, and in the case of two objects per image, that two separate islands form; one island is formed per object. 

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{figs/glom-examplefig.pdf}
    \caption{Examples of the results of the three experiments.
    A) 2-Basic: The randomly chosen objects happen to be a face and a sheep. GLOM reconstructs the whole nearly exactly.
    B) 1-Large: Two randomly chosen objects out of the twenty randomly created ones. GLOM is able to reconstruct, and separate the objects nearly perfectly.
    C and D) Perturbations of the 2-Basic experiment: The perturbed ellipses are given as input. The ellipses are nearly predicted correctly, and although there is more disagreement about the whole than in 2-Basic and 1-Large, there is still general agreement.  }
    \label{fig:example_outputs}
\end{figure}


\begin{comment}
\begin{figure}
    \centering
    \begin{tabular}{l|l|l|l|l|l}
        & & Classification & Element & Ellipse & Parameter \\
        & & Accuracy & MSE & MSE & Count \\ \hline
        2 Object Types, & MLP Baseline & 1.0 & 0.00053902 & 0.00076821 & 4,528,308 \\
        2 Per Image & GLOM & 1.0 & 0.0000096213 & 0.0000075917 & 2,322,554 \\ \hline
        20 Object Types, & MLP Baseline & 0.99656 & 0.010389 & 0.0049252 & 5,464,736 \\ 
        1 Per Image & GLOM & 1.0 & 0.000026012 & 0.000012101 & 2,025,343 \\
    \end{tabular}
    
    \caption{Baseline MLP vs GLOM for two cases. First, two random objects, each either a face or a sheep, containing five ellipses. Second, a single random shape, selected from a twenty randomly generated shapes, each containing five ellipses. The ellipses for each shape are ordered such that the ellipses are always given in the same ordering (ie. first the two eyes, then the mouth, etc).}
\end{figure}
\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
         & \multicolumn{3}{c}{2-Basic}                            & \multicolumn{3}{c}{1-Large}       \\ \midrule
         & Whole MSE  & Part MSE   & \multicolumn{1}{l|}{Params}  & Whole MSE  & Part MSE   & Params  \\
Baseline & 5.3 e^{-4} & 7.6 e^{-4} & \multicolumn{1}{l|}{4.5 e^6} & 1.0 e^{-2} & 4.9 e^{-3} & 5.4 e^6 \\
GLOM     & 9.6 e^{-6} & 7.5 e^{-6} & \multicolumn{1}{l|}{2.3 e^6} & 2.6 e^{-5} & 1.2 e^{-5} & 2.0 e^6 \\ \bottomrule
\end{tabular}
\label{tab:glom_vs_baseline_table}
\caption{Baseline MLP vs GLOM for two cases. First, two random objects, each either a face or a sheep, containing five ellipses. Second, a single random shape, selected from a twenty randomly generated shapes, each containing five ellipses. The ellipses for each shape are ordered such that the ellipses are always given in the same ordering (ie. first the two eyes, then the mouth, etc).}
\end{table}

There are multiple features of the network that can be modified to change the performance. This includes things like the type of decoder activation function, the size of the decoder layers, whether attention is enabled, the weight of the attention parameter when combining features at the Object Embedding level, the attention temperature, how the encoder/decoder features are combined at Ellipse Embedding level and Ellipse Symbol level (whether 'history' is considered, the weight of encoder vs decoder, whether it changes over iterations), the size of the embedding spaces, how the losses are combined (weighting of Object Loss vs Reconstruction Loss), and the number of iterations.

There are, additionally, a number of parameters we do not tune, but which affect performance. These include the grid size and other aspects of the datasets, such as the range of randomizations used to generate the random object instances.

We can consider seven different general areas of ablations: decoder (Fig. ~\ref{fig:decoder_variations}), combination functions (Fig. ~\ref{fig:combination_variations}), embedding spaces(Fig. ~\ref{fig:embedding_variations}), attention(Fig. ~\ref{fig:attention_variations}), iterations(Fig. ~\ref{fig:iteration_variations}), and loss combination(Fig. ~\ref{fig:loss_variations}). 

There is also the training procedure to consider. The Adam optimizer is used, with two parameters: initial learning rate and learning rate decay. 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{decoder_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary (independently) the decoder activation function and size of decoder layers. }
    \label{fig:decoder_variations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{combination_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary the history weight, and the top-down end weight. }
    \label{fig:combination_variations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{attention_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary the attention temperature, and the attention weight.}
    \label{fig:attention_variations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{embedding_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary the embedding size.}
    \label{fig:embedding_variations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{iteration_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary the number of iterations.}
    \label{fig:iteration_variations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{loss_variations}
    \caption{Chart/Table that shows variation of Classification Accuracy, Reconstruction Mean-Squared-Error, and Object Mean-Squared-Error as we vary the weight of the Reconstruction Loss vs Object Loss. When too much weight is given to the Reconstruction Loss, islands do not form. When too much weight is given to the Object Loss, there is a drift in the Ellipse Symbols, and the reconstruction mse suffers.}
    \label{fig:loss_variations}
\end{figure}

\paragraph{Analysis}

There are a couple questions we can ask: what is happening in the embedding, and how does it change over time?

The first question can be answered by looking at correlations in the embedding space and various parameters of the Object and Ellipse spaces. This can be done with xy coordinates (Fig. ~\ref{fig:embedding_basis_xy}), scale (x and y) (Fig. ~\ref{fig:embedding_basis_scale}) and rotation (only one rotation parameter) (Fig. ~\ref{fig:embedding_basis_rot}). 

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{embedding_basis_xy}
    \caption{Starting with the an Embedding Level from a model that had size, calculate the orthonormal basis (using X object examples as input). Then, calculated the x,y of the Object Symbol (or the Ellipse Symbol if operating on the Ellipse Embedding level), and plotted these x,y with the colour as the projection of the embedding onto one of the orthonormal basis vectors (the basis vectors are indexed here by their 'importance'/'weight' - as SVD is used to compute the orthonormal basis). Several "interesting" basis vectors are shown.
    This is shown for the Object Embedding and Ellipse Embedding.  }
    \label{fig:embedding_basis_xy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{embedding_basis_scale}
    \caption{Similar to Fig. ~\ref{fig:embedding_basis_xy}, but where we measure the correlation of the basis vector with scale instead of xy location. }
    \label{fig:embedding_basis_scale}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{embedding_basis_rot}
    \caption{Similar to Fig. ~\ref{fig:embedding_basis_xy}, but where we measure the correlation of the basis vector with rotation instead of xy location. }
    \label{fig:embedding_basis_rot}
\end{figure}

Alternatively, we can see that if we modify a single Object Embedding value, and use the encoder to go up to the Object Symbol, we can see how the object moves/changes once visualized. In this way, we can see that there are definitely correlations between different embedding values and the object type, location, rotation, scale, etc. (Fig. ~\ref{fig:embedding_modification})

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{embedding_modification}
    \caption{Modify a single Object Embedding value, and see how that modification changes the output Object Symbol. }
    \label{fig:embedding_modification}
\end{figure}

Finally, we can use T-SNE to visualize the embedding spaces over the iterations (Fig. ~\ref{fig:tsne_ellipse_object}). It shows that as it progresses through iterations, the two objects separate - sometimes both in the ellipse embedding level as well as the object embedding level. In cases where the object classification is not performed as well, we can see that the embedding spaces do not separate as well (Fig. ~\ref{fig:tsne_object_not_separated}).

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{tsne_ellipse_object}
    \caption{T-SNE can be used to embed the embedding spaces into a two dimensions, so we can see how it changes over iterations.}
    \label{fig:tsne_ellipse_object}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{tsne_object_not_separated}
    \caption{A t-sne plot showing that when the object symbols are confused at prediction time, it tends to also be confused at the object embedding level.}
    \label{fig:tsne_object_not_separated}
\end{figure}

When an additional regularizer is added, it can be seen that there is more separation between the two objects (Fig. ~\ref{fig:tsne_object_regularizer}).

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{tsne_object_regularizer}
    \caption{A t-sne plot showing the difference an additional regularizer makes.}
    \label{fig:tsne_object_regularizer}
\end{figure}

\paragraph{Robustness To Outliers / Noisy Inputs}

We can perturb the input ellipses slightly, and test whether the network can reconstruct the corrected ellipses and the correct objects. 

Additionally, we can provide data only within certain ranges of rotation, and show that in inference time, it is able to generalize to an angle it has never seen before.


